Memory-Efficient Community Detection on Large Graphs Using Weighted Sketches

Community detection in graphs identifies groups of nodes with denser connections within the groups than between them, and while existing studies often focus on optimizing detection performance, memory constraints become critical when processing large graphs on shared-memory systems. We recently proposed efficient implementations of the Louvain, Leiden, and Label Propagation Algorithms (LPA) for community detection. However, these incur significant memory overhead from the use of collision-free per-thread hashtables. To address this, we introduce memory-efficient alternatives using weighted Misra-Gries (MG) sketches, which replace the per-thread hashtables, and reduce memory demands in Louvain, Leiden, and LPA implementations - while incurring only a minor quality drop (up to 1%) and moderate runtime penalties. We believe that these approaches, though slightly slower, are well-suited for parallel processing and could outperform current memory-intensive techniques on systems with many threads.

==> src/alg-choose.tex <==
\begin{algorithm}[hbtp]
\caption{Choose the best community.}
\label{alg:choose}
\begin{algorithmic}[1]
\Require{$G(V, E)$: Input graph}
\Require{$C$: Community membership of each vertex}

\Statex

\Function{chooseBest}{$G, C$}
  \State $w_d \gets 0$
  \State $\rhd$ Compute total edge weight to communities
  \ForAll{$(j, w) \in G.edges(i)$}
    \If{\textbf{exclude self} $= 1$ \textbf{and} $i = j$} \textbf{continue} \label{alg:populate--exclude-self}
    \EndIf
    \If{\textbf{is refine phase and} $C_B[i] \neq C_B[j]$} \textbf{continue} \label{alg:populate--check-refine}
    \EndIf
    \State $c \gets C[j]$
    \If{$c = d$} $w_d \gets w_d + w$
    \EndIf
    \ForAll{$p \in [0, k)$}
      \State $S_v[p] \gets S_v[p] + w$ \textbf{if} $S_k[p] = c$ \textbf{else} $S_v[p]$
    \EndFor
  \EndFor
  \State $\rhd$ Choose community with best delta modularity
  \State $c^* \gets \phi$
  \State $\Delta Q^* \gets 0$
  \ForAll{$p \in [0, k)$}
    \If{$S_v[p] = 0$} \textbf{continue}
    \EndIf
    \State $\Delta Q \gets deltaModularity(S_v[p], w_d, K[i], \Sigma[S_k[p]], \Sigma[d], M)$
    \If{$\Delta Q > \Delta Q^*$}
      \State $c^* \gets S_k[p]$
      \State $\Delta Q^* \gets \Delta Q$
    \EndIf
  \EndFor
  \Return $[c^*, \Delta Q^*]$ \label{alg:choose--return}
\EndFunction
\end{algorithmic}
\end{algorithm}

